A new rule for almost-certain termination of probabilistic- and demonic programs

Extending our own and others' earlier approaches to reasoning about termination of probabilistic programs, we propose and prove a new rule for termination with probability one, also known as "almost-certain termination". The rule uses both (non-strict) super martingales and guarantees of progress, together, and it seems to cover significant cases that earlier methods do not. In particular, it suffices for termination of the unbounded symmetric random walk in both one- and two dimensions: for the first, we give a proof; for the second, we use a theorem of Foster to argue that a proof exists. Non-determinism (i.e. demonic choice) is supported; but we do currently restrict to discrete distributions.

==> Termination arXiv 170106/Macros.tex <==
% For TeXshop: make it LaTeX the root file if you cmt-T here.
% !TEX root = Termination.tex

% This winnowed from MacrosMaths 23 August 2016.

%%% CHECK WHAT'S ALREADY HERE BEFORE YOU ADD ANYTHING NEW :-)
%%% Probably you just need to un-comment an existing definition.

\newcommand\Abs[1]		{|#1|}
%\newcommand\ACapty[3]	{\mathcal{L}^+_{#2}(#3,#1)} 
\renewcommand\AC			{\textit{AC}} % Where is it previously defined?
\newcommand\ACT			{\textit{ACT}}
%\newcommand\AllOne		{{\mathbb O}} % So called because it's a right-zero for multiplication.
%\newcommand\AT			{@} % For `` with probability''.
%\newcommand\Atimes		{\times} % Arithmetic multipication of scalars,
%\newcommand\Ato[1]		{^{@#1}} % Probability of element in distribution enumeration.
%\newcommand\Att[2]		{^{@\nicefrac{#1}{#2}}} % Probability of element in distribution enumeration.
%\newcommand\Avg 		{{\sf avg}}
%\newcommand\AVG 		{\mathop\mu}
%\newcommand\basicgain[1]	{\cal{E}#1}
%\newcommand\BoldS {\mbox{\boldmath$S$}}
%\newcommand\Bool			{\mathit{Bool}}
%\newcommand\cala			{\mathcal{A}}	% Adversary
%\newcommand\calc			{\mathcal{C}}	% Contexts
%\newcommand\call			{\mathcal{L}}	% Leakage
%\newcommand\calml			{\mathcal{ML}} % Maximum Leakage, or Capacity
%\newcommand\cals			{\Spc{S}}
%\newcommand\calu			{\Spc{U}}
%\newcommand\calw			{\Spc{W}}	% Space of guesses
%\newcommand\calx			{\Spc{X}}	% Space of hidden inputs
%\newcommand\caly			{\Spc{Y}}	% Space of observable outputs
%\newcommand\calz			{\Spc{Z}}	% Another space of observable outputs
%\newcommand\CComp		{\mathbin{\parallel}}
%\newcommand\CDist[1]		{|\!| #1 |\!|_C}
%\newcommand\ChanHyp[2]	{[\Joint{#1}{#2}]} % The hyper you get by "multiplying" a prior into a channel.
%\newcommand\ChPar[2]		{#1{\parallel}#2}
%\newcommand\CloseSem		{]\!]}
%\newcommand\Col[2]		{#1_{-,#2}} % Dash for "all rows".
%\newcommand\Chi {\raisebox{.15em}{$\chi$}}
\newcommand\Comp		{\mathbin{\circ}} % Functional composition.
%\newcommand\Consonant {\textsc{cons}}
%\newcommand\DE[1]			{\DistEnum{#1}} % Shortcut.
\newcommand\Defs			{{:=}\,}
%\newcommand\Dem[1]		{#1^\sqcap}
%\newcommand\DemRef		{\mathrel{\Ref_\sqcap}}
\newcommand\Dist			{{\mathbb D}}
%\newcommand\DistA[1]		{{\mathbb D}{#1}} % With an argument.
%\newcommand\DistEnum[1]	{[#1]}
%\newcommand\Early {\textsc{early}}
%\newcommand\End 			{\hfill$\Box$}
%\newcommand\EQV			{eqv.}
\newcommand\Exp			{{\cal E}}
%\newcommand\Expec[2]		{{\cal E}_{#1}{#2}} % Expected value.
%\newcommand\Expt[2]		{{\cal E}_{#1}\,#2} % Expected value.
%\newcommand\FA			{{\forall}} % To enable/disable explicit forall symbol in capacities.
\newcommand\False			{\textit{false}}
%\newcommand\finitegain[1]	{\cal{G}#1}
\newcommand\Fun			{\mathbin{\rightarrow}} % Make it an operator to get correct spacing.
%\newcommand\GAdd[2]		{#1_{+#2}}
%\newcommand\GAddX[3]		{#1_{+#2@#3}} 
%\newcommand\GainFunc[1]	{{\mathbb	G}#1} % By analogy with other type-condstructors like \Dist.
%\newcommand\Gets			{{:=}\,}
%\newcommand\GMult[2]		{#1_{\times#2}}
%\newcommand\GVul[2]		{V_{#2}{#1}} % Backwards because the g-test is a postcondition.
%\newcommand\Hyp			{{\mathbb H}}
%\newcommand\HypA[1]		{{\mathbb D}^2{#1}} % With an argument.
%\newcommand\Iff			{\Leftrightarrow}
%\newcommand\Imp			{\Rightarrow}
\newcommand\Implies		{\mathbin{\Rightarrow}} % Proper spacing for binary operator.
\newcommand\In			{{:}\,} % Careful spacing for ":" meaning "is of type".
%\newcommand\Input			{\mbox{$\cal I$}} % Channel input.
%\newcommand\Inter			{\mathbin{\cap}}
%\newcommand\IS[3]			{#1[#2=+#3]}
%\renewcommand\Join		{\mathrel{\sqcup}} % \Join defined in some package.
%\newcommand\Joint[2]		{#1\rangle#2} % For discussion: should it be a more asymmetric symbol than comma?
%\newcommand\KantDist[1]		{|\!| #1 |\!|_K}
%\newcommand\KDist[3]		{{\mathbb K}_{#3}(#1,#2)} % Kantorovich distance
%\newcommand\Ker			{\mathop{\rm ker}}
%\newcommand\Knows		{\textsf{K}}
%\newcommand\Late 		{\textsc{late}}
\newcommand\Lgg			{\mathop{\textrm{lgg}}}
%\newcommand\lhs			{\textit{lhs}	}
%\newcommand\Lift[1] {#1^\ast\kern-.1em}
%\newcommand\LiftBox		{\vspace{-1em}} % Avoid extra space when display ends environment.
%\newcommand\Lipschitz[1]	{{\cal	L}^1#1} % Lipschitz property
%\DeclareMathSymbol\LLeftarrow{\mathrel}{AMSa}{"57}
%\newcommand\LMat[3]		{\makebox[0pt]{\raisebox{#2}[0pt][0pt]{$\left(\rule{0pt}{#3}\right.\hspace{#1}$}}}
\newcommand\Max			{\mathbin{\textsf{max}}}
%\newcommand\MCapty[3]		{\mathcal{L}_{#2}(#3,#1)}
%\newcommand\Meet			{\mathrel{\sqcap}}
%\newcommand\MFun			{\mathbin{\rightarrowtriangle}}
\newcommand\Min			{\mathbin\textsf{min}}
%\newcommand\MMult		{\mathbin{\cdot}} % Matrix multiplication.
%\newcommand\Mod			{\mathbin{\rm mod}}
%\newcommand\Nat			{{\mathbb N}}
%\newcommand\Natural		{\mathbb N}
%\newcommand\ND			{\mathbin{\sqcap}}
\newcommand\NF[2]			{\nicefrac{#1}{#2}}
\newcommand\NNReal		{{\mathbb R}^\geq}
%\newcommand\Norm[1]		{\lfloor#1\rfloor} % Normalisation of a distribution.
%\newcommand\NotDemRef	{\mathrel{\not\Ref_\sqcap}}
%\newcommand\NotPrbRef		{\mathrel{\not\Ref_\#}}
%\newcommand\NotPRef		{\mathrel{\not\preccurlyeq}}
%\newcommand\NotRef		{\mathrel{\not\sqsubseteq}}
%\newcommand\Nrm			{{\sf nrm}}
%\newcommand\Num[1]		{#1^{\textrm{\scriptsize\#}}}
%\newcommand\OpenSem		{[\![}
%\newcommand\Output		{\mbox{$\cal O$}} % Channel output.
%\newcommand\Part			{{\mathbb E}}
\newcommand\PC[1]			{\mathbin{{}_{#1}\kern-.05em\oplus}}
\newcommand\PCF			{\PC{\NF{1}{2}}}
\newcommand\pGCL		{\textit{pGCL}}
%\newcommand\Point[1]		{[#1]} % Point distribution or hyper.
\newcommand\Pow			{{\mathbb P}}%\kern-.05em}
%\newcommand\PowSq {\Pow^{\kern.07em2}\kern-.1em}
%\newcommand\PrbRef		{\mathrel{\Ref_\#}}
%\newcommand\PRef			{\mathrel{\preccurlyeq}}
\newcommand\Progress		{\emph{progress}}
%\newcommand\Rational		{\mathbb Q}
\newcommand\Real			{\mathbb R} % Real numbers
%\newcommand\Ref			{\mathrel\sqsubseteq}
%\newcommand\RESP		{resp.} % 1532.
%\newcommand\RevealAll[1]	{\textit{RevealAll}(#1)}
%\newcommand\rhs			{\textit{rhs}}
%\newcommand\RMat[3]		{\makebox[0pt]{\raisebox{#2}[0pt][0pt]{$\hspace{#1}\left.\rule{0pt}{#3}\right)$}}}
%\newcommand\Row[2]		{#1_{#2,-}} % Dash for "all columns".
%\newcommand\RRef			{\mathrel\sqsupseteq}
\DeclareMathSymbol\RRightarrow{\mathrel}{AMSa}{"56}
%\newcommand\Sc {\kern-.1em;\,}
%\newcommand\Sem[1]		{\OpenSem#1\CloseSem}
%\newcommand\SfA {\textsf{A}}
%\newcommand\SfB {\textsf{B}}
%\newcommand\SfE {\textsf{E}}
%\newcommand\Sfj {\textsf{j}}
%\newcommand\SfJ {\textsf{J}}
%\newcommand\Sfs {\textsf{s}}
%\newcommand\SfS {\textsf{S}}
%\newcommand\SfW {\textsf{W}}
%\newcommand\Size[1]		{|#1|}
%\newcommand\Skip			{\textit{Skip}}
%\newcommand\Smallsum[1]	{\textstyle{\sum_{#1}\:}} % Another less aggressive version.
\newcommand\SMart 		{\emph{super-martingale}}
%\newcommand\Spc[1]		{{\cal #1}} % Select font for input- or output space.
%\newcommand\Spot			{\mathbin{\mbox{\scriptsize$\bullet$}}} % 1144.
%\newcommand\SRef			{\mathrel{\sqsubset}}
%\newcommand\State			{\calx} % State space.
%\newcommand\StrictRef		{\mathrel\sqsubset}
%\newcommand\Sum[1]		{\Sigma#1} % Less aggressive symbol than \sum.
%\newcommand\Supp[1]		{\lceil#1\rceil} % Support of a distribution.
%\newcommand\Tau			{\textsf{T}}
\newcommand\True			{\textit{true}}
%\newcommand\Ucl			{{\mathbb U}}
%\newcommand\UClose[1]		{#1^{\Union}}
%\newcommand\Union		{\mathbin{\cup}}
%\newcommand\UNION		{\mathop\cup}
%\newcommand\VDist			{\overline{{\mathbb D}}}
%\newcommand\VHyp			{\overline{{\mathbb H}}}
%\newcommand\Vowel		{\textsc{vowel}}
\newcommand\VSRW		{V_\mathit{R}}
%\newcommand\WDist[3]		{{\mathbb W}_{#3}(#1,#2)} % Wasserstein distance
%\newcommand\Weight[1]		{\langle#1\rangle} % Weight of a partial distribution.
%\newcommand\WIDE[1]		{\Wide{\Wide{#1}}} % Extra wide space.
\newcommand\Wide[1] 		{~~~#1~~~} % Basic space.
%\newcommand\WIDERM[1]	{\Wide{\WideRm{#1}}} % Extra wide space around text.
\newcommand\WideRm[1]	{~~~\textrm{#1}~~~} % Basic space, but around text.
%\newcommand\WLOG		{wlog.} % 1532: Don't forget \ afterwards.
\newcommand\WLP			{\textsf{wlp}}
\newcommand\WP			{\textsf{wp}}
%\newcommand\WPROB		{wprob.} % 1532.
%\newcommand\WRT		{wrt.} % 1532.
%\newcommand\X[1] {\mbox{\Xx #1}} % Program.
%\newcommand\Xx			{\tt % Program-text font.
%\newcommand\DistEnum[1]	{\{\kern-.2em\{#1\}\kern-.2em\}}
%\newcommand\Spot		{\mathbin{\mathbold{\cdot}}} % 1144:The mathbold doesn't seem to work.

%\newcounter{Enums} % For run-on enumerations.
%\newenvironment{ReCorollary}[2]	{\par\textit{Corollary \ref{#2}:~}\textit{#1}\rm\quad}{\hfill$\Box$}
%\newenvironment{ReLemma}[2]		{\par\textit{Lemma \ref{#2}:~}\textit{#1}\rm\quad}{\hfill$\Box$}
%\newenvironment{ReTheorem}[2]	{\par\textit{Theorem \ref{#2}:~}\textit{#1}\rm\quad}{\hfill$\Box$}

%\newcommand\Joint[2] {[#1,#2]} % The joint you get by "multiplying" a prior into a channel.
%\newcommand\Lipshitz[1]{{\cal L}^1(#1)} % Misspelled.
%\newcommand\Abs[1] {#1^{\textrm{\scriptsize?}}}








==> Termination arXiv 170106/MacrosGeneral.tex <==
% For TeXshop: make it LaTeX the root file if you cmt-T here.
% !TEX root = Termination.tex

%%% MacrosGeneral 1 August 2016. 

%%% Our packages
%

\usepackage{amsfonts}			% For \mathbb.
\usepackage{amsmath}			% For \text.
\usepackage{amssymb}
\usepackage{bbding}				% For the small pencil.
\usepackage{chapterbib}			% For per-chapter references
\usepackage{endnotes}			% For endnotes.
\usepackage{enumerate}			% For custom enumerations.
\usepackage{graphicx}			% Including pictures etc.
\usepackage{hyperref}			% For allowing hyperlinks.
\usepackage{listings}			% 0923: For programs and ASCII: see environments for that.
\usepackage{longtable}			% For tables that go over pages.
\usepackage{stmaryrd}			% For the parallels.
\usepackage{subfigure}			% Small figures combined into one.
\usepackage[normalem]{ulem}		% For strikethroughs.
\usepackage{units}				% For \nicefrac.
\usepackage{url}				% For allowing urls.
\usepackage{wasysym}			% For \smiley and \hexagon.
\usepackage{wrapfig}
\usepackage{xcolor}				% For colours.

%\usepackage{amscd}
\usepackage{latexsym}
%\usepackage{mathrsfs}
%\usepackage{txfonts}			% For the (temporary) refinement symbol.
%\usepackage{verbatim}


%%% Assorted extras

% http://tex.stackexchange.com/questions/32597/vertically-centered-horizontal-rule-filling-the-rest-of-a-line
\def\Vhrulefill{\leavevmode\leaders\hrule height 0.7ex depth \dimexpr0.4pt-0.7ex\hfill\kern0pt}


%%% Graphic helper
%

% \ImageInText{upNudge}{rightNudge}{scaleFactor}{fileName}
\newcommand\ImageInText[4]%
{\makebox[0pt][l]{%
{\def\Up{#1}\def\Right{#2}% Use \def in case they're already defined.
\hfill%
\raisebox{\Up}[0pt][0pt]{% No height, no depth.
\makebox[0pt][l]{\hspace{\Right}% No width.
\includegraphics[scale=#3]{#4}%
}}}}}

% \ImageInTextBlock{height}{depth}{width}{upNudge}{rightNudge}{scaleFactor}{fileName}
\newcommand\ImageInTextBlock[7]%
{\def\Height{#1}% Use \def in case they're already defined.
 \def\Depth{#2}
 \def\Width{#3}
 \def\Up{#4}
 \def\Right{#5}
\raisebox{\Up}[\Height][\Depth]{
\makebox[\Width][l]{\hspace{\Right}
\includegraphics[scale=#6]{#7}%
}}}


%%% Theorems, figures, footnotes etc.
%

% These already defined by Springer.
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{lemma}[theorem]{Lemma}

\newcommand\FirstLineOfTheorem[1][\empty] {\ifx#1\empty\quad\else~\hrulefill~#1\\\fi}
\newcommand\MakeFact[2]{\newenvironment{#1}[2]{\begin{#2}\label{##2}\textit{##1}\rm\noexpand\noexpand\FirstLineOfTheorem}{\hfill$\Box$\end{#2}}}

\MakeFact{Definition}{definition}
\MakeFact{Corollary}{corollary}
\MakeFact{Lemma}{lemma}
\MakeFact{Theorem}{theorem}

% In case we want a uniform change.
\newenvironment{Figure}[2] {\begin{figure}\def\z{#1}\def\zz{#2}\small}{\caption{\makebox[0em][r]{\raisebox{.2em}{\rule{2em}{.05em}}\hspace{5.5em}}\quad\zz\quad\raisebox{.2em}{\rule{2em}{.05em}}}\label{\z}\end{figure}}

\newcommand\Chapter[1]{\chapter{#1}}
\newcommand\Section[1]{\section{#1}}
\newcommand\Subsection[1]{\subsection{#1}}
\newcommand\Subsubsection[1]{\subsubsection{#1}}

% \Footnote[]{xxx} closes up 0.1em.
% \Footnote{xxx} is as normal..
% \Footnote[<length>]{xxx} closes up <length>.
% http://tex.stackexchange.com/questions/127502/difference-between-if-and-ifx
\newcommand\Footnote[2][\empty] {\ifx#1\empty\kern-0.1em\else\if*#1\relax\else\kern-#1\fi\fi\footnote{#2}} 

% Helpers for referring to them.
\newcommand\Cor[1] {Cor.~\ref{#1}}
\newcommand\Chp[1] {Chap.~\ref{#1}}
\newcommand\Def[1] {Def.~\ref{#1}}
\newcommand\Eqn[1] {(\ref{#1})}
\newcommand\Lem[1] {Lem.~\ref{#1}}
\newcommand\Thm[1] {Thm.~\ref{#1}}
\newcommand\Sec[1] {\S\ref{#1}}
\newcommand\App[1] {App.~\ref{#1}}
\newcommand\Fig[2][\empty] {\ifx#1\empty Fig.~\ref{#2}\else Fig.~\ref{#2}(#1)\fi}
\newcommand\Note[1] {\FnSym\ref{#1}}
\newcommand\Itm[1] {(\ref{#1})}
\newcommand\Itms[2] {(\ref{#1}--\ref{#2})}
\newcommand\Pg[1] {p.\pageref{#1}}
%
% Proof -- is it a part of the theorem, or not?
% That is, do we write
%
    %Theorem
    %	statement of theorem
    %END_THEOREM
    %Proof
    %	details of proof
    %END_PROOF
%
% or do we write
%
    %Theorem
    %	statement of theorem
    %Proof
    %	details of proof
    %END_MATHS
%
%\newcommand\Proof{\par\noindent\textit{Proof:}\quad}
\newenvironment{Proof}{\par\smallskip\noindent\textbf{Proof}\quad}{}%~\hfill$\Box$}

%%% 0923: Environments for typesetting ASCII text and program text
%

% See http://tex.stackexchange.com/questions/11973/verbatim-environment-and-line-breaking
\lstnewenvironment{Prog} {
	\lstset{
		language=csh,
		basicstyle=\ttfamily,	% 1350: Should agree with \PF, i.e. program font.
  		breaklines=false,	% 0922: Don't wrap lines in Prog.
  		showspaces=false,
  		keywords={vis,hid,var,while,if,end,begin,to,then,fi,leak},
  		columns=flexible,
  		escapechar=\%,	% 0920: Use "%" for escape to LaTeX, since it doesn't work as comment in verbatim anyway.
  		mathescape=true
	}
}{}

\newenvironment{ProgFrags}{ % For inline program fragments, delimited both sides by "!" .
	\lstMakeShortInline[
		language=csh,
		basicstyle=\ttfamily,	% 1350.
  		breaklines=false,	% 0922.
  		showspaces=false,
  		keywords={vis,hid,var,while,if,end,begin,to,then,fi,leak},
  		columns=flexible,
  		escapechar=\%,	% 0920. But doesn't work in-line?
  		mathescape=true
	]!
}
{\lstDeleteShortInline!}

\lstnewenvironment{ASCII} {
	\lstset{
		language=csh,
		basicstyle=\ttfamily,
  		showspaces=false,
  		breaklines=true,	% 0922: Wrap lines in ASCII.
  		breakindent=0pt,
  		keywords={},
  		columns=flexible,
  		escapechar=\%,	% 0920.
  		mathescape=true
	}
}{}

\newenvironment{EqnText}[1] {\begin{equation}\label{#1}\begin{minipage}{0.8\linewidth}}{\end{minipage}\end{equation}}

%%% Here's two toy examples: the first creates a "quote like" display, with no number and therefore no way of referring to it. The second makes an "equation like" display, with a label.

% Inside "Prog" you can escape to LeTeX with %stuff% and escape to maths with $maths$. Obviously "%" doesn't work as comment in that case.

% No number, no label.
%	\newcommand\Leak {print} % We have't decided whether to call it "leak", or "print" or "reveal".
%	\begin{Prog}
%	x:= 0;
%	y:= 1 $\PC{\nicefrac{1}{2}}$ 2;
%	if x=0 then
%		while y=2 do
%			%\Leak% 0 ${\ND}$ (x+y)
%		end
%	fi
%	\end{Prog}

% With number and label. Unfortunately, I cannot manage to combine the \begin{EqnText}\begin{Prog} into a single \begin{Something}.
% On the other hand, EqnText can be used more generally when you want an equation-like reference to something that isn't maths:
% it doesn't have to have Prog inside.

%	\begin{EqnText}{e1234}
%	\begin{Prog}
%	x:= 0;
%	y:= 1 $\PC{\nicefrac{1}{2}}$ 2;
%	if x=0 then
%		while y=2 do
%			%\Leak% 0 ${\ND}$ (x+y)
%		end
%	fi
%	\end{Prog}
%	\end{EqnText}


%%% Macros for equational reasoning
%
\newenvironment{Reason}{\begin{tabbing}\hspace{4em}\= \hspace{1cm} \= \kill}
    {\end{tabbing}\vspace{-1em}}
\newcommand\Step[2] {#1 \> $\begin{array}[t]{@{}llll}#2\end{array}$ \\}
\newcommand\StepR[3] {#1 \> $\begin{array}[t]{@{}llll}#3\end{array}$
    \` {\RF \makebox[0pt][r]{\begin{tabular}[t]{r}``#2''\end{tabular}}} \\}
\newcommand\WideStepR[3] {#1 \>
    $\begin{array}[t]{@{}ll}~\\#3\end{array}$ \`
    {\RF \makebox[0pt][r]{\begin{tabular}[t]{r}``#2''\end{tabular}}} \\}
\newcommand\Space {~ \\}
\newcommand\RF {\small}

%%% Here's a toy example:

%	\begin{Reason}
%	\Step{}{ % First step has no operator and no reason.
% 		first expression
%	}
%	\StepR{$=$}{because it's equal}{ % Second step is related to first by =, and has a reason. Note $$.
% 		second expression
%	}
%	\Space % Blank line before and after multi-line steps: this one's before.
% 	% Third step is related to second by if, and has a long reason. Not no $$.
%	\WideStepR{$=$}{because it's equal, equal, equal, equal, equal, equal, equal, equal, equal, equal, equal, equal, }{
% 		third expression
%	}
%	\Space % This one's after.
%	\Step{$\Implies$}{ % Last step ends with $\quad$ and some punctuation, if it makes sense grammatically
% 		fourth expression \quad.
%	}
%	\end{Reason}

%%% Here's a real example from CSF14 p10.
% 	Note there's no colon before, and a comma afterwards. The grammar is thus the same as if we had written
%
%	Thus we calculate $(x+1)^2=x^2+2x+1$, whence the result follows...
%
%

%	Thus we calculate
%	\begin{Reason}
%	\Step{}{
%		\WDist{\Point{\pi}}{\ChanHyp{\pi}{{C}}}{\Hyp{\Spc{X}}} 
%	}
%	\StepR{$=$}{$d$ is underlying metric; \Def{d0636}}{
% 		\min_{S\In\Spc{S}_{\Sigma,\Tau}} \Expec{S}{d}
%	}
%	\StepR{$=$}{take unique $S$ in $\Spc{S}$ as at \Eqn{e1314}}{
% 		\Expec{S}{d}
%	}
%	\Space
%	\StepR{$=$}{define $d_\sigma(\tau)\Defs d(\sigma,\tau)$ to allow Currying;\\
%            $S$ at \Eqn{e1314} has point left-marginal $\Point{\pi}$}{
% 		\Expec{\ChanHyp{\pi}{{C}}}{d_\pi}
%	}
%	\Space
%	\StepR{$=$}{define $g$ so that $\GVul{\Point{\tau}}{g} = d_\pi(\tau){+}1$; see below}{
%		\GVul{\ChanHyp{\pi}{{C}}}{g} - 1
%	}
%	\StepR{$=$}{$\GVul{\Point{\pi}}{g} = d_\pi(\pi){+}1 = 1$}{
%		\GVul{\ChanHyp{\pi}{{C}}}{g} - \GVul{\Point{\pi}}{g}
%	}
%	\StepR{$\leq$}{\Def{d0730}}{
%		\ACapty{{C}}{\FA}{\pi}
%	}
%	\StepR{$\leq$}{\Lem{l1411}}{
%		\KDist{\Point{\pi}}{\ChanHyp{\pi}{{C}}}{\Hyp{\Spc{X}}} ~,
%	}
%	\end{Reason}
%	whence the result follows because we have sandwiched $\ACapty{{C}}{\FA}{\pi}$
%	between $\WDist{\Point{\pi}}{\ChanHyp{\pi}{{C}}}{\Hyp{\Spc{X}}}$
%	and $\KDist{\Point{\pi}}{\ChanHyp{\pi}{{C}}}{\Hyp{\Spc{X}}}$
%	--- which from \Thm{t0647} are equal.
        


==> Termination arXiv 170106/MacrosLabels.tex <==
% For TeXshop: make it LaTeX the root file if you cmt-T here.
% !TEX root = Termination.tex

%%% Label hints --- 1720: Has to be called after the (Springer) \begin{document}, which resets \label.
%%% Also it doesn't seem to work inside of \begin{equation}, which also resets \label.
%%% Carroll Morgan 3 August 2016
%

\newif\ifShowLabels
\newcommand\SL[1] {\mbox{\tt\scriptsize[#1]}}
\newcommand\LabelWithShow[1] {\ifShowLabels\ifinner\SL{#1}\else\ifmmode\SL{#1}\else\marginpar{\SL{#1}}\fi\fi\fi\Label{#1}}
\let\Label\label \let\label\LabelWithShow

\newcommand\ShowLabels {\ShowLabelstrue} % Put labels in the margin for convenience.
\newcommand\NoShowLabels {\ShowLabelsfalse} % Don't do that.

% Kludge to get around Springer's re-redefining \label inside \Begin{Equation}.
% Later could replace equation with Equation "behind the scenes"; but for now just use \begin{Equation} directly if you want this feature.
% See http://latex-community.org/forum/viewtopic.php?f=45&t=23165
\newif\ifShowLabelsWas
\newenvironment{Equation}{\ShowLabelsWasfalse\ifShowLabels\ShowLabelsWastrue\begin{equation}\let\LabelWas\Label\let\Label\label\let\label\LabelWithShow\else\begin{equation}\fi}{\end{equation}\ifShowLabelsWas\let\label\Label\let\Label\LabelWas\fi\ShowLabelsWasfalse}

==> Termination arXiv 170106/MacrosMarkup.tex <==
% For TeXshop: make it LaTeX the root file if you cmt-T here.
% !TEX root = Termination.tex

%%% Macros for "in progress" artefacts: colours, funny footnotes, funny endnotes, showing labels etc.
%%% MacrosMarkup Carroll Morgan 30a August 2016

\usepackage{amssymb}			% For \boxtimes.
\usepackage[normalem]{ulem}		% For strikethroughs.
\usepackage{bbding}				% For the small pencil.
%\usepackage{dingbat}			% For pointing hand.
\usepackage{endnotes}			% For endnotes.
\usepackage{hyperref}			% For hyperlinks to and from endnotes.

%%% Colours and markups
%
\definecolor{PurplePlum}{rgb}{0.1,0,0.55} 
\definecolor{Brown}{rgb}{0.5,.25,0}
\definecolor{Orange}{rgb}{1,.6,0}
\definecolor{Gray}{rgb}{.7,.7,.7}
\definecolor{DarkGreen}{rgb}{0,.6,0}

%\definecolor{Black}{rgb}{0,0,0}
%\definecolor{PineGreen}{rgb}{0,0.5,0.5}
%\definecolor{Green}{rgb}{0,.5,0}

\newif\ifBleck
\newcommand\Bleck {\Blecktrue} % Carry out all deletes and replacements; remove all footnotes/endnotes; make everything black.
% To check that all colouring-calls to markup functions have been removed, disable \Bleck and enable Colour->\undef.

\newcommand\Colour[1] {\color{#1}}
%\renewcommand\Colour[1] {\undef} % Enable this to check that no colours are used by Markups.

% http://tex.stackexchange.com/questions/201348/why-doesnt-makeatletter-work-inside-newcommand
\newcommand\ToCLinks {
 \ifBleck\else % 1031: Put hyperlink to ToC  and GR at bottom of every page.
   \expandafter\def\csname@oddfoot\endcsname{
    {\Colour{blue}\mbox{\hyperlink{w1619}{\sf$\rightarrow$~top}\quad
    				    \hyperlink{w1031}{\sf$\rightarrow$~toc}\quad
                                      \hyperlink{GreenRoom}{\sf$\rightarrow$~gr}\quad
                                      \hyperlink{EndNotes}{\sf$\rightarrow$~en}\quad
                                      \hyperlink{Sargasso}{\sf$\rightarrow$~sg}}\hfill
   }}
   % Can't get \let to work here.
   \expandafter\def\csname@evenfoot\endcsname{
    {\Colour{blue}\mbox{\hyperlink{w1619}{\sf$\rightarrow$~top}\quad
                                      \hyperlink{w1031}{\sf$\rightarrow$~toc}\quad
                                      \hyperlink{GreenRoom}{\sf$\rightarrow$~gr}\quad
                                      \hyperlink{EndNotes}{\sf$\rightarrow$~en}\quad
                                      \hyperlink{Sargasso}{\sf$\rightarrow$~sg}}\hfill
   }}
 \fi
}

\newif\ifEndNotes % 0831: Workaround for endnotes-bug: missing ".ent" file when there are no endnotes.

\newcommand\FnSym{{\scriptsize\PencilLeftDown\kern.1em}} % Needs bbding.
\newcommand\EnSym {{$\bigtriangledown$}}
\newcommand\Fn[1] {[\FnSym\ref{#1}]} % For referring to footnotes.
\newcommand\En[1] {[\EnSym\ref{#1}]} % For referring to EndNotes.
\newcommand\ENSection[1] {\par\noindent\textbf{\large #1}\par\medskip}
\newcommand\ENSubsection[1] {\par\noindent\textbf{#1}\par\medskip}
\newcommand\ENItem[1] {\item[\textbf{#1}]~\par}
%\newcommand\Later {(\C{later})}
%\newcommand\NA[1] {{\Colour{#1}\large\phone}~}

%%%  \MakeMarkups[optionalComment]{prefixLetter}{textModifier}
%%%  One for each person: for example C for prefixLetter and \Colour{blue} for textModifier would be
%%%
%%%     \MakeMarkups[optionalComment]{C}{\Colour{blue}}
%%%
%%%  A possible use for optionalComment is to give the person's name.
%%%
%%%  "Disabling" a markup (or all of them) makes the document look as if that (those) markups had
%%%  been carried out. Replacements/deletions are done; footnotes, endnotes and t-comments are
%%%  removed; the document becomes black.
%%%
%%%  Disable all markups with macro \Bleck; also Green Room, Sargasso and Endnotes are suppressed.
%%%  Disable individual markup (rather than all via \Bleck) by eg \MakeMarkups[0]{C}{...}
%%%  Re-enable individual markups in spite of \Bleck with \MakeMarkups[1]{C}{...}
%%%

\newif\ifMakeMarkupsCalled %1121: Print help text only once.
\newif\ifSuppress % Whether to suppress these annotations.
\newcommand\MakeMarkups[3][.]{%1119
 \Suppressfalse % Suppress these markups if (Bleck OR [0]) and not [1].
 \ifBleck\Suppresstrue\fi
 \ifx0#1\Suppresstrue\fi
 \ifx1#1\Suppressfalse\fi
%
 \expandafter\providecommand\csname#2x\endcsname {} % 1613: This trick allows MakeMarkups to be called more than once for a particular person.
 \ifSuppress\expandafter\renewcommand\csname#2x\endcsname{\relax}\else
                   \expandafter\renewcommand\csname#2x\endcsname{#3}\fi % \Xx: Change to colour.
% 
 \expandafter\providecommand\csname#2\endcsname {} % 1613.
 \ifSuppress\expandafter\renewcommand\csname#2\endcsname[1]{##1}\else
                   \expandafter\renewcommand\csname#2\endcsname[1]{{\csname#2x\endcsname##1}}\fi % \X{#1}: Put #1 in colour.
%
 \expandafter\providecommand\csname#2d\endcsname {} % 1613.
 \ifSuppress\expandafter\renewcommand\csname#2d\endcsname[1]{\relax}\else
                   \expandafter\renewcommand\csname#2d\endcsname[1]{{\csname#2x\endcsname\sout{##1}}}\fi % \Xd{#1}: Delete (strikeout) #1; needs ulem package.
%
 \expandafter\providecommand\csname#2r\endcsname {} % 1613.
 \ifSuppress\expandafter\renewcommand\csname#2r\endcsname[2]{{##2}}\else
                   \expandafter\renewcommand\csname#2r\endcsname[2]{\csname#2d\endcsname{##1} \csname#2\endcsname{##2}}\fi % \Xr{#1}{#2}: Replace #1 with #2.
%
 \expandafter\providecommand\csname#2t\endcsname {} % 1613.
 \ifSuppress\expandafter\renewcommand\csname#2t\endcsname[1]{\relax}\else
                   \expandafter\renewcommand\csname#2t\endcsname[1]{{\csname#2x\endcsname{$\langle\!\langle$##1$\rangle\!\rangle$}}}\fi % \Xt{#1}: Like \Xd{#1} but without strikeout; use where \Xf{#1} not allowed.
%
 \expandafter\providecommand\csname#2b\endcsname {} % 1613.
 \ifSuppress\expandafter\renewcommand\csname#2b\endcsname[1][\empty]{\relax}\else % \Xb[#1]: Put bookmark in the margin, with optional parameter.
                   \expandafter\renewcommand\csname#2b\endcsname[1][\empty]{\ifx##1\empty
                   	\label{#2-bookmark} % With hyperlinks you can jump directly to your bookmark by clicking on an appropriate \pageref.
                          \marginpar [\raggedleft\csname#2\endcsname{{\footnotesize\fbox{#2 working here}}~$\Longrightarrow$}]
                                            {\csname#2\endcsname{$\Longleftarrow$~{\footnotesize\fbox{#2 working here}}}}
                   \else % No label if there's an explicit parameter.
                   	% In general \ifx#1\empty\empty succeeds if the argument #1 is \empty, or begins with \empty\empty or is actually empty:
			% in the first case \if gets true for #1=\empty, and evaluates the second \empty to empty;
			% in the second case it gets true for \empty=\empty (in #1), and evaluates the following \empty\empty to empty;
			% and in the third case it gets true for \empty=\empty.
			% Anything else gives false.
                   	\marginpar [\raggedleft\csname#2\endcsname{\ifx##1\empty\empty\else\fbox{\tiny\parbox{8em}{\raggedright##1}}~\fi$\Longrightarrow$}]
                                            {\csname#2\endcsname{$\Longleftarrow$\ifx##1\empty\empty\else~{\tiny\fbox{\parbox{8em}{\raggedright##1}}}\fi}}\fi}\fi
%
 \expandafter\providecommand\csname#2TD\endcsname {} % 1613.
 \ifSuppress\expandafter\renewcommand\csname#2TD\endcsname{\relax}\else
                   \expandafter\renewcommand\csname#2TD\endcsname{\csname#2\endcsname{\fbox{\texttt{#2} to do}}}\fi % \XTD: This person to do.
%
 \expandafter\providecommand\csname#2Bar\endcsname {} % 1613.
 \ifSuppress\expandafter\renewcommand\csname#2Bar\endcsname{\relax}\else
                   \expandafter\renewcommand\csname#2Bar\endcsname{\csname#2\endcsname{\scriptsize\XSolidBrush}}\fi % \XBar: Left by other people: delete when you're happy.
%
% \Xf{#1}: Make coloured "footnote #1 to self".
 \expandafter\providecommand\csname#2f\endcsname {} % 1613.
 \ifSuppress\expandafter\renewcommand\csname#2f\endcsname[2][]{\relax}\else
  \expandafter\renewcommand\csname#2f\endcsname[2][\empty]{ % Have forgotten what the optional parameter was for.
    {\mbox{\csname#2x\endcsname\tiny$\boxtimes$}\marginpar{\csname#2x\endcsname\fbox{\FnSym\footnotemark}}\relax 
    \footnotetext{\csname#2x\endcsname##2}}}\fi
%
% \Xe{#1}: An endnote: like \Xf, but longer text #1 put at the end of the document.
 \expandafter\providecommand\csname#2e\endcsname {} % 1613.
 \ifSuppress\expandafter\renewcommand\csname#2e\endcsname[1]{\relax}\else
  \expandafter\renewcommand\csname#2e\endcsname[1]{
   \EndNotestrue %0831
   \mbox{\scriptsize\csname#2x\endcsname$\boxtimes$}\relax
   \marginpar{\csname#2x\endcsname\fbox{\EnSym\endnotemark
                      \hypertarget{ENmark\thepage-\theendnote}{}~\hyperlink{ENtext\thepage-\theendnote}{{\Colour{blue}$\downarrow$}}}
   }
   { % 1641 Make \z,\zz local.
    \def\zz{\noexpand#3}
    \edef\z{~{\zz[Endnote \theendnote\ on p.\noexpand\hypertarget{ENtext\thepage-\theendnote}{}\thepage
                ~\noexpand\hyperlink{ENmark\thepage-\theendnote}{{\noexpand\Colour{blue}$\uparrow$}}]}
    }
    \expandafter\endnotetext\expandafter{\z\vspace{2ex}\\ ##1\newpage}
   } %1641
  }\fi
%  
% Like \Xf and \Xe together --- Use \Xfe[<file name for endnote>]{Short footnote about file's contents.}
 \expandafter\providecommand\csname#2fe\endcsname {} % 1613.
 \ifSuppress\expandafter\renewcommand\csname#2fe\endcsname[2][]{\relax}\else %1538
  \expandafter\renewcommand\csname#2fe\endcsname[2][]{ % 1540: \File is local.
   \def\File{##1}\relax
   \ifx\File\empty\csname#2f\endcsname{##2}\else % 1536: Without file, behave like \Xf.
    \EndNotestrue %0831
    \mbox{\scriptsize\csname#2x\endcsname$\boxtimes$}
    \marginpar{\csname#2x\endcsname\fbox{\FnSym\footnotemark}}\relax
    \footnotetext{~\csname#2x\endcsname##2\
                         --- See [\EnSym\endnotemark\hypertarget{ENmark\thepage-\theendnote}{}
                         \kern-.2em\hyperlink{ENtext\thepage-\theendnote}{{\Colour{blue}$\downarrow$}}].}\relax
   { % 1641 Make \z,\zz local.
     \def\zz{\noexpand#3}
     \edef\z{~{\zz[Footnote~\thefootnote~on~p.\noexpand\hypertarget{ENtext\thepage-\theendnote}{}\thepage
                 ~\noexpand\hyperlink{ENmark\thepage-\theendnote}
                 {{\noexpand\Colour{blue}\kern-0.1em$\uparrow$}]}}
                 {\noexpand\footnotesize\noexpand\newline\noexpand\hspace*{2em} (~from file {\noexpand\tt\File.tex}~)}
     }    
     \expandafter\endnotetext\expandafter{\z~\par\input{##1}\newpage}
    } %1641
   \fi % 1536
  } % 1540
 \fi % 1538
%
% "How-to" material printed by the first call to \MakeMarkups; suppress by \MakeMarkupCalledtrue just before that first call.
 \ifSuppress\relax\else%0749
  \csname#2f\endcsname{%1009
   $\backslash$\texttt{#2}$\cdots$\ markups are in \textbf{this} colour\ifx#1..\else\ifx1#1.\else, for #1.\fi\fi
   \ifMakeMarkupsCalled\relax\else %1121
    \begin{quote}\begin{tabular}{l@{\hspace{2em}}p{.8\linewidth}}
     \multicolumn{2}{l}{\texttt{$\backslash$MakeMarkups\ifx#1.\relax\else[#1]\fi\{#2\}\{{\it$\langle$colour command\/$\rangle$}\}}
     				 --- Defines the macros below:}\\
         & see comments at \texttt{$\backslash$MakeMarkups} definition. \\[1ex]
     \texttt{$\backslash$#2\{$\langle$text$\rangle$\}} & Sets \texttt{$\langle$text$\rangle$} in \texttt{#2}'s colour. \\
     \texttt{$\backslash$#2x} & Changes to \texttt{#2}'s colour (until end of context). \\
     \texttt{$\backslash$#2d\{$\langle$text$\rangle$\}} & Sets \texttt{$\langle$text$\rangle$} in \texttt{#2}'s colour with a strikethrough (i.e.\ delete). \\
     \texttt{$\backslash$#2r\{$\langle$this$\rangle$\}\{$\langle$that$\rangle$\}} &
      Strikes through \texttt{$\langle$this$\rangle$} and inserts \texttt{$\langle$that$\rangle$} (i.e.\ replace). \\
     \texttt{$\backslash$#2f\{$\langle$text$\rangle$\}} & Meta-comment: puts \texttt{$\langle$text$\rangle$} in a \texttt{#2}-footnote with a {\tiny$\boxtimes$} in the main text. \\
     \texttt{$\backslash$#2t\{$\langle$text$\rangle$\}} & Use for meta when  \texttt{$\backslash$#2f} isn't allowed (``Not in outer-par mode.'') \\
     \texttt{$\backslash$#2b[$\langle$optional$\rangle$]} & Marginal pointer, with label for hyper-linking directly there. \\
     \texttt{$\backslash$#2e\{$\langle$text$\rangle$\}} & Puts \texttt{$\langle$text$\rangle$} in a \texttt{#2}-endnote with a (big) $\boxtimes$ in the main text. \\[.5ex]
     \texttt{$\backslash$#2fe[$\langle$this$\rangle$]\{$\langle$that$\rangle$\}} & Makes a  \texttt{$\backslash$#2f\{$\langle$that$\rangle$\}} that refers to a \\
       & \texttt{$\backslash$#2e\{$\langle$contents of file this.tex$\rangle$\}}. \\ 
       & Without the optional argument, acts as \texttt{$\backslash$#2f\{$\langle$that$\rangle$\}}. \\[.5ex]
     \texttt{$\backslash$#2Bar} & Inserts ``burn after reading'' symbol \csname#2Bar\endcsname, meaning
      \begin{quote}\begin{itemize}\setlength\itemsep{0pt}
       \item If yours is the only \csname#2Bar\endcsname\ in this (presumably someone else's) footnote, and you are happy that the footnote has been addressed,
       go ahead and comment-out the whole footnote. (The \csname#2Bar\endcsname\ is their request for you to ``approve and remove''.)
       \item If you are not happy, delete only your \csname#2Bar\endcsname\ and follow-on in the footnote
        (in your colour, i.e.\ with \texttt{$\backslash$#2x}) saying why you are not happy.
       \item If you are happy, but there are others' burn-after-reading symbols as well as yours, just delete yours; the other people have not yet responded.
      \end{itemize}
      \end{quote}
      The idea is that when everyone's happy, the last person will comment-out the meta-text. \\[0.5ex]
     \texttt{$\backslash$#2TD} & Inserts {\csname#2TD\endcsname}\ . \\
    \end{tabular}\end{quote}
   \fi
  }%1009
  \MakeMarkupsCalledtrue %1121
 \fi%0749
}%1119

\newcommand\Divider {~\vfill~\bigskip\hrule~\\\hrule~\bigskip} % For separating contributions in GreenRoom etc. Put in contributor's colour.
\newcommand\MakeGreenRoom {\ifBleck\relax\else
% \cleardoublepage % Not necessary if \include'd.
 \hrule
 ~\\\begin{center}\Huge \hypertarget{GreenRoom}{Green Room}
 \end{center}~\\
 \hrule
\fi}

\newcommand\MakeEndNotes {\ifBleck\relax\else
% \cleardoublepage % Not necessary if \include'd.
 \hrule~\\\begin{center}\ifEndNotes\Huge Endnotes\else\textit{No endnote macros were called in this run.}\fi\end{center}~\\\hrule
 {\parindent 0pt \parskip 2ex \def\enotesize{\normalsize} \def\notesname{} % Supress EndNotes title.
 \ifEndNotes\theendnotes\fi} %0831
\fi}

\newcommand\MakeSargasso {
 % Localise labels and references to Sargasso itself, if possible.
 % Stuff In Sargasso might be a copy of earlier material, and we don't want the earlier labels to be overwritten.
 \hypertarget{Sargasso}{}
 \newcommand\NewLabel[1] {\OldLabel{Sargasso-##1}} % All Sargasso labels "branded".
 \newcommand\NewRef[1] % All Sargasso references take branded version if possible.
 {\expandafter\ifx\csname r@Sargasso-##1\endcsname\relax\OldRef{##1}\else\OldRef{Sargasso-##1}\fi}
 % Now swap them over.
 \let\OldLabel\label \let\label\NewLabel
 \let\OldRef\ref \let\ref\NewRef
 %
 \ifBleck\end{document}\else
% \cleardoublepage % Not necessary if \include'd.
  \hrule
  ~\\\begin{center}\Huge Sargasso
  \end{center}~\\
  \hrule
 \fi
}

% For citations to be filled-in later: better than \cite{later} because \cite{later} generates undefined-reference warnings that might mask real ones.
% \Cite is -not- disabled by \Bleck, since \Bleck is supposed to make a version that is "OK to submit", and missing references is not "not OK".
% If necessary however (eg in a panic :-) you can enable \Bleck and disable \Cite, the latter by uncommenting the command following.
\newcommand\Cite[2][\empty] {{\color{red}\ifx#1\empty[#2]\else[#2,~#1]\fi}}
%\renewcommand\Cite[1] {\relax}

%%% End of \Markups

